Opto-Electronic Characterization of Three Dimensional Topological Insulators

We demonstrate that the terahertz/infrared radiation induced photogalvanic effect, which is sensitive to the surface symmetry and scattering details, can be applied to study the high frequency conductivity of the surface states in (Bi1-xSbx)2Te3 based three dimensional (3D) topological insulators (TI). In particular, measuring the polarization dependence of the photogalvanic current and scanning with a micrometre sized beam spot across the sample, provides access to (i) topographical inhomogeneity's in the electronic properties of the surface states and (ii) the local domain orientation. An important advantage of the proposed method is that it can be applied to study TIs at room temperature and even in materials with a high electron density of bulk carriers.

==> references_APL.tex <==


\begin{thebibliography}{99}

	\bibitem{HasanKane2010} M. Z. Hasan and C. L. Kane, 
	%Colloquium: Topological insulators,
	Rev. Mod. Phys. \textbf{82}, 3045 (2010).
	
	\bibitem{Moore2010} J. E. Moore, 
	%The birth of topological insulators,
	Nature \textbf{464}, 194 (2010).
	
	\bibitem{QiZhang2011}  X. L. Qi and S. C. Zhang,
	%Topological insulators and superconductors,
	Rev. Mod. Phys. \textbf{83}, 1057 (2011).
	
	\bibitem{Bardarson2013} J. H. Bardarson and J. E. Moore, 
	%Quantum interference and Aharonov?ohm oscillations in topological insulators
	Rep. Prog. Phys. \textbf{76}, 056501 (2013). 
	
	\bibitem{Bernevig2013} B. A. Bernevig, 
	\textit{Topological Insulators and Superconductors}
	(University Press Group Ltd, 2013).
	
	% % % % %SURFACE DOMINANT TRANPORT % % % % % % %
	
	\bibitem{bulk_states1} J. G. Checkelsky, Y. S. Hor, M. H. Liu, D. X. Qu, R. J. Cava, and N. P. Ong,
	%Quantum interference in macroscopic crystals of nonmetallic Bi2Se3,
	Phys. Rev. Lett. \textbf{103}, 246601 (2009).
	
	\bibitem{bulk_states2} A. A. Taskin and Y. Ando,
	%Quantum oscillations in a topological insulator Bi1?xSbx,
	Phys. Rev. B \textbf{80}, 085303 (2009).
	
	\bibitem{bulk_states3}  J. G. Analytis, J. H. Chu, Y. Chen, F. Corredor, R. D. McDonald, Z. X. Shen, and I. R. Fisher,
	%Bulk Fermi surface coexistence with Dirac surface state in Bi2Se3: A comparison of photoemission and Shubnikov–de Haas measurements,
	Phys. Rev. B \textbf{81}, 205407 (2010). 
	
	\bibitem{MBE_1} L. He, X. Kou, K. L. Wang, 
	Phys. Status Solidi RRL \textbf{7}, 50 
	%–63, %No. 1–2, DOI 10.1002/pssr.201307003
	(2013).
	
	\bibitem{MBE_2} G. Wang, X.-G. Zhu, Y.-Y. Sun, Y.-Y. Li, T. Zhang, J. Wen, X. Chen, K. He, L.-L. Wang, X.-C. Ma, J.-F. Jia, S. B. Zhang, and Q.-K.  Xue, 
	Adv. Mater. \textbf{23}, 2929 (2011).
	% DOI: 10.1002/adma.201100678
	
	\bibitem{MBE_3} J. Krumrain, G. Mussler, S. Borisova, T. Stoica, L. Plucinski, C. M. Schneider, and D. Grützmacher, 
	J. Crystal Growth \textbf{324}, 115  (2011).
	%,   DOI: 10.1016/j.jcrysgro.2011.03.008 
	
	\bibitem{MBE_4} S. E. Harrison, S. Li, Y. Huo, B. Zhou, Y. L. Chen, and J. S. Harris
	Appl. Phys. Lett. \textbf{102}, 171906 (2013).
	%; doi: 10.1063/1.4803717
	
	\bibitem{transport1}  T. C. Hsiung, C. Y. Mou, T.K. Lee, and Y. Y. Chen
	%Surface-dominated transport and enhanced thermoelectric figure of merit in topological insulator Bi1.5Sb0.5Te1.7Se1.3 
	Nanoscale \textbf{7}, 518 (2015).
	
	\bibitem{transport2}  J. Yong, Y. P. Jiang, D. Usanmaz, S.  Curtarolo, X. H. Zhang, L. Z. Li, X. Q.  Pan, J.  Shin, I. Takeuchi, and R. L. Greene
	%Robust topological surface state in Kondo insulator SmB6 thin films 
	Appl. Phys. Lett. \textbf{105}, 222403 (2014).
	
	\bibitem{transport3} T. C. Hsiung, D. Y. Chen, L.  Zhao, Y. H.  Lin, C. Y.  Mou, T. K.  Lee, M. K.  Wu, and Y. Y. Chen
	%Enhanced surface mobility and quantum oscillations in topological insulator Bi1.5Sb0.5Te1.7Se1.3 nanoflakes 
	Appl. Phys. Lett \textbf{103}, 163111 (2013).
	
	\bibitem{transport4} B. Xia, P. Ren, A. Sulaev, P. Liu, S. Q.  Shen, and L. Wang
	%Indications of surface-dominated transport in single crystalline nanoflake devices of topological insulator Bi1.5Sb0.5Te1.8Se1.2 
	Phys. Rev. B \textbf{87}, 085442 (2013).
	
	\bibitem{transport5} Z. Ren, A. A.  Taskin, S.  Sasaki, K. Segawa, and Y. Ando
	%Fermi level tuning and a large activation gap achieved in the topological insulator Bi2Te2Se by Sn doping 
	Phys. Rev. B. \textbf{85}, 155301 (2012).
	
	\bibitem{transport6} L. He, F. X.  Xiu, X. X.  Yu, M. Teague, M W. J. Jiang, Y. B.  Fan, X. F.  Kou, M. R. Lang, Y.  Wang, G.  Huang, N. C.  Yeh, and K. L. Wang
	%Surface-Dominated Conduction in a 6 nm thick Bi2Se3 Thin Film 
	Nano Lett. \textbf{12}, 1486 (2012).
	
	\bibitem{Barreto2014} L. Barreto, L. K\"{u}hnemund, F. Edler, Ch. Tegenkamp, J. Mi, M. Bremholm, B. B. Iversen, Ch. Frydendahl, M. Bianchi, and P. Hofmann
	%Surface-Dominated Transport on a Bulk Topological Insulator
	Nano Lett. \textbf{14}, 3755
	%−3760
	(2014).
	
	\bibitem{Ren2010} Z. Ren, A. A. Taskin, S. Sasaki, K. Segawa, and Y. Ando
	%Large bulk resistivity and surface quantum oscillations in the topological insulator Bi2Te2Se
	Phys. Rev. B \textbf{82}, 241306(R) (2010).
	
	\bibitem{Qu2010} D.-X. Qu, Y. S. Hor, J. Xiong, R. J. Cava, N. P. Ong
	%Quantum Oscillations and Hall Anomaly of Surface States in the Topological Insulator Bi2Te3
	Science \textbf{329}, 821 (2010).
	
	\bibitem{Trans_doped1} C.-Z. Chang, J. Zhang, X. Feng, J. Shen, Z. Zhang, M. Guo, K. Li, Y. Ou, P. Wei, L.-L. Wang, Z.-Q. Ji, Y. Feng, S. Ji, X. Chen, J. Jia, X. Dai, Z. Fang, S.-C. Zhang, K. He, Y. Wang, L. Lu, X.-C. Ma, and Q.-K. Xue
	%Experimental Observation of the Quantum Anomalous Hall Effect in a Magnetic Topological Insulator
	Science  \textbf{340}, 6129 (2013).
	
	\bibitem{Trans_doped2} C.-Z. Chang, W. Zhao, D. Y. Kim, H. Zhang, B. A. Assaf, D. Heiman, S.-C. Zhang, C. Liu, M. H. W. Chan, and  J. S. Moodera
	%High-precision realization of robust quantum anomalous Hall state in a hard ferromagnetic topological insulator
	Nature Materials \textbf{14}, 473
	%–477
	(2015).
	
	\bibitem{Trans_doped3} A. J. Bestwick, E. J. Fox, X. Kou, L. Pan, K. L. Wang, and D. Goldhaber-Gordon
	%Precise Quantization of the Anomalous Hall Effect near Zero Magnetic Field
	Phys. Rev. Lett. \textbf{114}, 187201 (2015).
	
	\bibitem{Trans_doped4} A. Kandala,  A. Richardella,  S. Kempinger,  C.-X. Liu, and N. Samarth
	%Giant anisotropic magnetoresistance in a quantum anomalous Hall insulator
	Nat. Comm. \textbf{6}, 7434 (2015).
	
	% % % % % % % % ARPES XRD SEM % % % % % % % %
	\bibitem{ARPES_2} Y. Xia, D. Qian, D. Hsieh, L. Wray, A. Pal, H. Lin, A. Bansil, D. Grauer, Y. S. Hor, R. J. Cava, and M. Z. Hasan,
	%Observation of a large-gap topological-insulator class with a single Dirac cone on the surface,
	Nature Physics \textbf{5}, 398 (2009).
	
	\bibitem{ARPES_3}  D. Hsieh, Y. Xia, D. Qian, L. Wray, J. H. Dil, F. Meier, J. Osterwalder, L. Patthey, J. G. Checkelsky, N. P. Ong, A. V. Fedorov, H. Lin, A. Bansil, D. Grauer, Y. S. Hor, R. J. Cava, and M. Z. Hasan,
	%A tunable topological insulator in the spin helical Dirac transport regime,
	Nature (London) \textbf{460}, 1101 (2009).
	
	\bibitem{ARPES_5} Y. L. Chen, J. G. Analytis, J.-H. Chu, Z. K. Liu, S.-K. Mo, X. L. Qi, H. J. Zhang, D. H. Lu, X. Dai Z. Fang, S. C. Zhang, I. R. Fisher, Z. Hussain, and Z.-X. Shen,
	%Experimental Realization of a Three-Dimensional Topological Insulator, Bi 2 Te 3
	Science \textbf{325}, 178 (2009).
	
	\bibitem{ARPES_1}  C. Chen, S. He, H. Weng, W. Zhang, L. Zhao, H. Liu, X. Jia, D. Mou, S. Liu, J. He, Y. Peng, Y. Feng, Z. Xie, G. Liu, X. Dong, J. Zhang, X. Wang, Q. Peng, Z. Wang, S. Zhang, F. Yang, C. Chen, Z. Xu, X. Dai, Z. Fang, and X. J. Zhou,
	%Robustness of topological order and formation of quantum well states in topological insulators exposed to ambient environment
	PNAS \textbf{109}, 3694 (2012).
	
	\bibitem{ARPES_6} Z.-H. Pan, E. Vescovo, A. V. Fedorov, G. D. Gu, and T. Valla,
	%Persistent coherence and spin polarization of topological surface states on topological insulators
	Phys. Rev. B \textbf{88}, 041101 (2013). 
	
	\bibitem{timeARPES} M. Hajlaoui, E. Papalazarou, J. Mauchain, Z. Jiang, I. Miotkowski, Y.P. Chen, A. Taleb-Ibrahimi, L. Perfetti, and M. Marsi
	%Time resolved ultrafast ARPES for the study of topological insulators: The case of Bi2Te3
	Eur. Phys. J. Special Topics \textbf{222}, 1271
	%–1275 
	(2013).
	
	\bibitem{ARPES_4}  Y. Liu,	Y. Y. Li,	S. Rajput,	D. Gilks,	L. Lari,	P. L. Galindo,	M. Weinert,	V. K. Lazarov, and L. Li
	%Tuning Dirac states by strain in the topological insulator Bi2Se3
	Nat. Phys. \textbf{10}, 294
	%–299 
	(2014).
	
	\bibitem{2ppe1} J.  Reimann, J.  Gudde, K.  Kuroda, E. V. Chulkov, and U. Hofer
	%Spectroscopy and dynamics of unoccupied electronic states of the topological insulators Sb2Te3 and Sb2Te2S
	Phys. Rev. B. \textbf{90}, 081106 (2014).
	
	\bibitem{2ppe3} S. Zhu, Y. Ishida, K. Kuroda, K. Sumida, M. Ye, J. Wang, H. Pan, M. Taniguchi, S. Qiao, S. Shin, and A. Kimura
	%Ultrafast electron dynamics at the Dirac node of the topological insulator Sb2Te3
	Scient. Rep. \textbf{5}, 13213 (2015).	
	
	\bibitem{2ppe2} K. Kuroda, J. Reimann, J. G\"{u}dde, and U. H\"{o}fer
	%Generation of Transient Photocurrents in the Topological Surface State of Sb2Te3 by Direct Optical Excitation with Midinfrared Pulses
	Phys. Rev. Lett. \textbf{116}, 076801 (2016).
	
	\bibitem{STM1} G. Zhang, H. Qin, J. Teng, J. Guo, Q. Guo, X. Dai, Z. Fang, and K. Wu
	%Quintuple-layer epitaxy of thin films of topological insulator Bi 2 Se 3
	Appl. Phys. \textbf{95}, 053114 (2009).
	
	\bibitem{STM2} Z.Y. Wang, H.D. Li,  X. Guo , W.K. Ho, and M.H. Xie
	%Growth characteristics of topological insulator Bi2Se3 films on different substrates
	J. Cryst. Growth \textbf{334}, 96 
	%-102
	(2011).
	
	\bibitem{STM3} Z. Alpichshev, R. R. Biswas, A. V. Balatsky, J. G. Analytis, J.-H. Chu, I. R. Fisher, and A. Kapitulnik
	%STM Imaging of Impurity Resonances on Bi2Se3
	Phys. Rev. Lett. \textbf{108}, 206402 (2012).
	
	\bibitem{Samarath}  A. Richardella, A. Kandala, J. Sue Lee, and N. Samarth
	%Characterizing the structure of topological insulator thin films
	Appl. Phys. Lett Mater \textbf{3}, 083303 (2015).
	
	\bibitem{SEM} M. Zhang, Z. Wei, R. Jin, Y. Ji, Y. Yan, X. Pu, X. Yang, and Y. Zhao, 
	Thin Solid Films \textbf{603}, 289 (2016). 
	%doi:10.1016/j.tsf.2016.02.043
	
	\bibitem{AFM} G. Bendt, S. Zastrow, K. Nielsch, P. S. Mandal, J. Sanchez-Barriga, O. Rader, and S. Schulz, 
	J. Mater. Chem. A, {\bf 2}, 8215 (2014).
	% DOI: 10.1039/c4ta00707g
	
	\bibitem{XRD} H. Cao, R. Venkatasubramanian, C. Liu, J. Pierce, H. Yang, M. Z. Hasan, Y. Wu, and Y. P. Chen, 
	Appl. Phys. Lett. {\bf 101}, 162104 (2012).
	%, DOI: 10.1063/1.4760226
	
	\bibitem{Hamh} S. Y. Hamh et al., 
	Appl. Phys. Lett., \textbf{108}  051609 (2016).
	
	\bibitem{Basov} B. C. Chapler, K. W. Post, A. R. Richardella, 
	J. S. Lee, J. Tao, N. Samarth, and D. N. Basov,
	%Infrared electrodynamics and ferromagnetism in the topological semiconductors Bi2Te3 and Mn-doped Bi2Te3
	Phys. Rev. B \textbf{89}, 235308 (2014).
	
	\bibitem{Loosdrecht}  N. Borgwardt, J. Lux, I. Vergara, Zhiwei Wang, A. A. Taskin, Kouji Segawa, P. H. M. van Loosdrecht, Y. Ando, A. Rosch, and M. Gr\"{u}ninger
	%Revealing puddles of electrons and holes in compensated topological insulators
	Phys. Rev. B, \textbf{93} 245149 (2016).
	
	% % % % % % % PHOTOCURRENTS % % % % % % % % %
	
	\bibitem{Ganichev2003} S. D. Ganichev and W. Prettl, 
	%Spin photocurrents in quantum wells,
	topical review, J. Phys.: Condens. Matter, \textbf{15}, R935 (2003).
	
	\bibitem{book} S. D. Ganichev and  W. Prettl, 
	\textit{Intense Terahertz Excitation of Semiconductors}
	(Oxford Univ. Press, Oxford, 2006).
	
	\bibitem{Olbrich2014} P. Olbrich, L. E. Golub, T. Herrmann, S.N. Danilov, H. Plank, V.V. Bel'kov, G. Mussler, Ch. Weyrich, C. M. Schneider, J. Kampmeier, D. Gr\"{u}utzmacher, L. Plucinski, M. Eschbach, and S. D. Ganichev, 
	%Room temperature high frequency transport of Dirac fermions in epitaxially grown Sb2Te3 and Bi2Te3-based topological insulators, 
	Phys. Rev. Lett. \textbf{113}, 096601 (2014).
	
	\bibitem{Kastl2015_1} Ch. Kastl, Ch. Karnetzky, H. Karl, and A. W. Holleitner, 
	%Ultrafast helicity control of surface currents in topological insulators with near-unity fidelity, 
	Nature Comm. \textbf{6}, 6617 (2015).
	
	\bibitem{Braun2015} L. Braun, G. Mussler, A. Hruban, M. Konczykowski, M. Wolf, T. Schumann, M. M\"{u}nzenberg, L. Perfetti, T. Kampfrath, 
	%Ultrafast shift photocurrents at the surface of the three-dimensional topological insulator Bi2Se3, 
	arXiv:1511.00482 (2015).
	
	\bibitem{Plank2016} H. Plank, L. E. Golub, S. Bauer, V.V. Bel’kov, T. Herrmann, P. Olbrich, M. Eschbach, L. Plucinski, C. M. Schneider, J. Kampmeier, M. Lanius, G. Mussler, D. Gr\"{u}tzmacher, and S. D. Ganichev
	%Photon drag effect in (Bi1-xSbx)(2)Te-3 three-dimensional topological insulators
	Phys. Rev. B \textbf{93}, 125434  (2016).
	
	\bibitem{Borisova2012} S. Borisova, J. Krumrain, M. Luysberg, G. Mussler, and D. Gr\"{u}tzmacher,
	%Mode of Growth of Ultrathin Topological Insulator Bi2Te3 Films on Si (111) Substrates,
	Cryst. Growth Des. \textbf{12}, 6098
	%-6103
	(2012).
	
	\bibitem{Plucinski2013} L. Plucinski, A. Herdt, S. Fahrendorf, G. Bihlmayer, G. Mussler, S. D\"{o}ring, J. Kampmeier, F. Matthes, D. E. Bürgler, D. Gr\"{u}tzmacher, S. Bl\"{u}gel, and C. M. Schneider, 
	%Electronic structure, surface morphology, and topologically protected surface states of Sb2Te3 thin ﬁlms grown on Si(111)
	Appl. Phys. \textbf{113}, 053706 (2013).
	
	\bibitem{Borisova2013} S. Borisova, J. Kampmeier, M. Luysberg, G. Mussler and D. Gr\"{u}tzmacher,
	%Domain formation due to surface steps in topological insulator Bi2Te3 thin films grown on Si (111) by molecular beam epitaxy
	Appl. Phys. Lett. \textbf{103}, 081902 (2013).
	
	%that the majority of the domains have the same orientation
	\bibitem{Kampmeier2015} J. Kampmeier, S. Borisova, L. Plucinski, M. Luysberg, G. Mussler, and D. Gr\"{u}tzmacher, 
	%Suppressing Twin Domains in Molecular Beam Epitaxy Grown Bi2Te3 Topological Insulator Thin Films
	Cryst. Growth Des., \textbf{15}, 390 (2015).
	%pp 390–394
	
	\bibitem{ternaries} C. Weyrich, M. Dr\"ogeler, J. Kampmeier, M. Eschbach, G. Mussler, T. Merzenich, T. Stoica, I. E. Batov, J. Schubert, L. Plucinski, B. Beschoten, C. M. Schneider, C. Stampfer, D. Gr\"utzmacher, and Th. Sch\"apers, 
	%Growth, characterization, and transport properties of ternary (Bi1−xSbx)2Te3 topological insulator layers
	arxiv 1511.00965v2 (2015).
	
	% % % % % % % % % technique % % % % % % % %
	
	\bibitem{removalSiGe}  
	%Removal of spin degeneracy in p-SiGe quantum wells demonstrated by spin photocurrents
	S.D. Ganichev et al., 
	%U. Rossler, W. Prettl, et al.
	Phys. Rev. B \textbf{66}, 075328   (2002). 
	%37
	
	\bibitem{Resonantinversion2003} S.D. Ganichev, V. V. Bel'kov, Petra Schneider, E. L. Ivchenko, S. A. Tarasenko,  W. Wegscheider, D. Weiss,    D. Schuh, E. V. Beregulin  and  W. Prettl, 
	%{\it Resonant inversion of circular photogalvanic effect in $n$-doped quantum wells,}\\
	Phys. Rev. B {\bf 68}, 035319 (2003).
	%37
	
	\bibitem{SGEopt2003} S. D. Ganichev, Petra Schneider, V. V. Bel'kov, E. L. Ivchenko, S. A. Tarasenko, W. Wegscheider, D. Weiss, D. Schuh, B. N. Murdin, P. J. Phillips,  C. R. Pidgeon, D. G. Clarke, M. Merrick,  P. Murzyn,  E. V. Beregulin, and W. Prettl,
	%{\it Spin galvanic effect due to optical spin orientation,}\\
	Phys. Rev. B. R {\bf 68}, 081302 (2003).
	%36+1
	
	\bibitem{Chongyun} 
	%Helicity-dependent photocurrents in graphene layers excited by midinfrared radiation of a CO2 laser
	Chongyun Jiang et a., 
	%, V.A. Shalygin, V.Yu. Panevin,  et al.
	Phys. Rev. B \textbf{84}, 125429   (2011).
	%24+1+1
	
	\bibitem{Lechner2009}
	%Tuning of structure inversion asymmetry by the delta-doping position in (001)-grown GaAs quantum wells
	V. Lechner, L. E. Golub, P. Olbrich, S. Stachel, D. Schuh, W. Wegscheider, V. V. Bel'kov, and S. D. Ganichev,
	%\textit{  Tuning of structure inversion asymmetry by the $\delta$-doping position in (001)-grown GaAs quantum wells},\\
	Appl. Phys. Lett. \textbf{94}, 242109 (2009).
	%28
	
	\bibitem{Drexler2013} C. Drexler,  S. A. Tarasenko, P. Olbrich, J. Karch, M. Hirmer, F. M\"{u}ller, M. Gmitra, J. Fabian, R. Yakimova, S. Lara-Avila, S. Kubatkin, and S. D. Ganichev,
	%\textit{Magnetic quantum ratchet effect in graphene}\\
	Nature Nanotechnology \textbf{8}, 104 (2013).
	%27
	
	\bibitem{ratchet2009} P. Olbrich, E. L. Ivchenko, T. Feil, R. Ravash, S. D. Danilov, J. Allerdings, D. Weiss, and S. D. Ganichev,
	%\textit{Ratchet effects induced by terahertz radiation in heterostructures with a lateral
	%periodic potential}\\
	Phys. Rev. Lett. \textbf{103}, 090603 (2009).
	%33
	
	\bibitem{helix2012} M. Kohda, V. Lechner, Y. Kunihashi, T. Dollinger, P. Olbrich, C. Sch\"{o}nhuber,  I. Caspers, V. V. Bel'kov, L. E. Golub, D. Weiss, K. Richter, J. Nittaand S. D. Ganichev,
	%\textit{Gate-controlled Persistent Spin Helix State in InGaAs quantum wells}\\
	Phys. Rev. B Rapid Communic. \textbf{86}, 081306 (2012).
	%26
	
	\bibitem{Ganichev84p20} S. D. Ganichev, Y. V. Terent'ev, and I. D. Yaroshetskii, 
	%%Photon-drag  photodetectors  for  the  far-IR  and  submillimeter regions
	Pisma Zh. Tekh. Fiz. \textbf{11}, 46 (1985) [Sov. Tech. Phys. Lett. \textbf{11}, 20 (1989)].
	
	%lambda
	\bibitem{BelkovSSTlateral} V. V. Bel'kov,  and S. D. Ganichev,
	%Magneto-gyrotropic effects in semiconductor quantum wells, review.
	Semicond. Sci. Technol. \textbf{23}, 114003 (2008).
	%33+1
	
	\bibitem{ratchet2011} P. Olbrich, J. Karch, E. L. Ivchenko, J. Kamann, B. M{\"a}rz, M. Fehrenbacher, D. Weiss, and S. D. Ganichev,
	%\textit{Classical ratchet effects in heterostructures with a lateral periodic potential}\\
	Phys. Rev. B \textbf{83}, 165320 (2011).
	%24+1
	
	%pyroelectric camera 
	\bibitem{Ganichev1999} S. D. Ganichev
	%\textit{Tunnel ionization of deep impurities in semiconductors induced by terahertz electric fields} \\
	Physica B \textbf{273-274}, 737 (1999).
	%37
	
	\bibitem{Ziemann2000}  E. Ziemann, S. D. Ganichev, I. N. Yassievich, V. I. Perel, and W. Prettl,
	%%Characterization of deep impurities in semiconductors by terahertz tunneling ionization
	J. Appl. Phys. {\bf 87}, 3843 (2000).
	%39
	
	\bibitem{NatPhys09} H. Zhang, C.-X. Liu, X.-L. Qi, X. Dai, Z. Fang, and S.-C. Zhang,
	%%Topological insulators in Bi2Se3, Bi2Te3 and Sb2Te3 with a single Dirac cone on the surface,
	Nature Phys. \textbf{5}, 438 (2009).
	
	% % % % FOOTNOTES % % % % % % % % %
	
	\bibitem{footnoteT1} Note that for quasi-elastic scattering by phonons we obtain the expression 
	which differs from the equation above by a constant factor of order of unity only.
	
	\bibitem{footnoteT3}
	Due to the fact that in the applied frequency range the 
	condition $\omega _{\rm tr}\tau \gg 1$ is satisfied we are limited 
	here to the statement that the room temperature mobility of the surface states 
	is at least higher that 1000\,cm$^2$/Vs. However, photogalvanic experiments in a 
	spectral range substantially extended to lower frequencies, e.g. applying Gunn diode or backwardwave
	oscillator, would allows one to measure the electron mobility.
	In this regime the LPGE photocurrent magnitude $A \propto \sigma(\omega)$
	will change its behaviour from $A~\propto (\omega\tau_{tr})^{-2}$ to the 
	frequency independent one:  a function allowing to obtain $\tau_{tr}$
	with rather high accuracy.
	
	\bibitem{footnoteT2} In the case contacts or edges are illuminated the signal becomes polarization independent and increases by three orders of magnitude compared to photogalvanic effect in middle part of the sample.  The assignment of this signal which can be caused 
	by e.g. $p-n$ junctions or thermal effects in inhomogeneous area close to contacts 
	is out of scope of this paper.
	
\end{thebibliography}


